RTGPU: Real-Time GPU Scheduling of Hard Deadline Parallel Tasks with Fine-Grain Utilization

Many emerging cyber-physical systems, such as autonomous vehicles and robots, rely heavily on artificial intelligence and machine learning algorithms to perform important system operations. Since these highly parallel applications are computationally intensive, they need to be accelerated by graphics processing units (GPUs) to meet stringent timing constraints. However, despite the wide adoption of GPUs, efficiently scheduling multiple GPU applications while providing rigorous real-time guarantees remains a challenge. In this paper, we propose RTGPU, which can schedule the execution of multiple GPU applications in real-time to meet hard deadlines. Each GPU application can have multiple CPU execution and memory copy segments, as well as GPU kernels. We start with a model to explicitly account for the CPU and memory copy segments of these applications. We then consider the GPU architecture in the development of a precise timing model for the GPU kernels and leverage a technique known as persistent threads to implement fine-grained kernel scheduling with improved performance through interleaved execution. Next, we propose a general method for scheduling parallel GPU applications in real time. Finally, to schedule multiple parallel GPU applications, we propose a practical real-time scheduling algorithm based on federated scheduling and grid search (for GPU kernel segments) with uniprocessor fixed priority scheduling (for multiple CPU and memory copy segments). Our approach provides superior schedulability compared with previous work, and gives real-time guarantees to meet hard deadlines for multiple GPU applications according to comprehensive validation and evaluation on a real NVIDIA GTX1080Ti GPU system.

==> old_sched.tex <==

\section{Practical RT-GPU Tasks Scheduling}
\label{sec:schedule}

In this section, we first introduce the task model for real-time GPU applications, then propose the RT-GPU scheduling algorithm, and develop the corresponding response time analysis. 
{\color{red} "Revise the brief intro of the RT-GPU algorithm:"\\
In our proposed algorithm, we will first use GPU kernel federated scheduling to determine the GPU response time and then propose a fixed priority scheduling algorithm for the full system. As far as we know, the proposed fixed priority scheduling achieves the best schedulability compared with state-of-the-art real-time scheduling algorithm for the similar systems and models. 
}


\begin{figure}
\centering
\includegraphics[width=0.48\textwidth]{scheduling_model}
\caption{GPU tasks real-time scheduling model.}
\label{fig:scheduling_model}
\vspace{-5mm}
\end{figure}


\subsection{Task Model}

%As discussed in Section \ref{sec:CPU_memory} and \ref{sec:GPU_model}, each GPU task has CPU segments, memory copy segments and GPU kernel segments, which must be executed in order. The CPU code executes logic operations serially and usually does not contain parallel execution inside one task. The memory movement from CPU (host) and GPU (device) is through a PCIe or network-on-chip interface in an explicit or implicit manner. Helped by the persistent technique with workload pinning, now the many-SM GPU can be used as a classic manycore system and the GPU kernel can be executed fully in parallel on specific SMs but the execution is in a non-preemptive manner \cite{GPUpreem}. 

%Based on previous discussion and system work, GPU tasks scheduling model is shown in Fig. \ref{fig:scheduling_model}. In this scheduling model, there is a preemptive CPU core executing the CPU segments, a non-preemptive communication interface (bus) for memory copy segments, a GPU with many cores (SMs) for the GPU kernels. This model is not limited to general commercial embedded, desktop and server GPU systems, it can also be appropriate for the general heterogeneous computing system such as CPU+FPGA, CPU+accelerator architectures and so on.

%Since the GPU tasks are embarrassingly parallel workloads and there is no synchronization between tasks

Leveraging the platform implementation and the resulted CPU, memory and GPU models just discussed, we formally define the parallel real-time tasks executing on a CPU-GPU platform. We consider a task set $\tau$ comprised of $n$ sporadic tasks, where $\tau = \{ \tau_1, \tau_2, \cdots, \tau_n \}$. Each task $\tau_i$, where $1\le i\le n$, has a relative deadline $D_{i}$ and a period (minimum inter-arrival time) $T_{i}$. In this work, we restrict our attention to constrained-deadline tasks where $D_i \leq T_i$. Moreover, task $\tau_i$ consists of $m_i$ CPU segments, $2m_i-1$ memory-copy segments, and $m_i-1$ GPU segments. 
As discussed in Section~\ref{kernelmodel}, a GPU segment $G_{i}^{j}$ models the execution of a GPU kernel on interleaved SMs using total work $\GW_{i}^{j}$, critical-path overhead $\GL_{i}^{j}$, and interleaved execution ratio $\alpha_{i}^{j}$, i.e., $G_{i}^{j} = (\GW_{i}^{j}, \GL_{i}^{j}, \alpha_{i}^{j} )$.
Thus, task $\tau_i$ can be characterized by the following 3-tuple:
\begin{equation}
\begin{split}
\tau_i = 
\Big( & \big(\CL_{i}^{0}, \ML_{i}^{0}, G_{i}^{0}, \ML_{i}^{1}, 
 \CL_{i}^{1}, \ML_{i}^{2}, G_{i}^{1}, \ML_{i}^{3}, \\ 
& \cdots, \CL_{i}^{j}, \ML_{i}^{2j}, G_{i}^{j}, \ML_{i}^{2j+1}, \cdots, 
 \CL_{i}^{m_{i}-2}, \\ & \ML_{i}^{2m_{i}-4}, G_{i}^{m_{i}-2}, \ML_{i}^{2m_{i}-3}, 
 \CL_{i}^{m_{i}-1} \big), D_{i}, T_{i} \Big)
\label{eq:intrinsic_Switched_capacitor_loss}
\end{split}
\end{equation}
where $\CL_{i}^{j}$ and $\ML_{i}^{j}$ are the execution times of the \mbox{$(j+1)$-th} CPU and memory-copy segments, respectively. In addition, we use $\widecheck{\ \ }$ and $\widehat{\ \ }$ to denote the lower and upper bound on a random variable. For example, $\CLup_{i}^{j}$ and $\CLlo_{i}^{j}$ are the upper and lower bounds on execution times of the $(j+1)$-th CPU segment of $\tau_i$, respectively.

%If ${m_{i}}$ is 1, there is only one CPU segment of $\tau_i$, and the task $\tau_i$ does not have memory copy or GPU codes. This model is a basic configuration where there is one CPU execution, one time memory movement and one GPU execution in one CPU, memory. and GPU data flow. Any task configurations can be generated from this configuration by setting the length of undesired segments to zero. A task system $\tau$ is said to be an implicit-deadline system if its deadline is equal to its period and a constrained-deadline system if the relative deadline of each task is no larger than its period.

{\color{red} Revise the def of response time: \\
Besides, $CR_{i}^{j}$, $MR_{i}^{j}$ and $GR_{i}^{j}$ are the response time of the corresponding CPU segment, memory segment and GPU segment, which ranges in intervals %$[{\mathop{CR_{i}^{j}}\limits^{\vee}_{}} \; {\mathop{CR_{i}^{j}}\limits^{\wedge}_{}}]$, 
%$[{\mathop{MR_{i}^{j}}\limits^{\vee}_{}} \; {\mathop{MR_{i}^{j}}\limits^{\wedge}_{}}]$, and 
%$[{\mathop{GR_{i}^{j}}\limits^{\vee}_{}} \; {\mathop{GR_{i}^{j}}\limits^{\wedge}_{}}]$,  
$[{\CRlo_{i}^{j}} \; {\CRup_{i}^{j}}]$, 
$[{\MRlo_{i}^{j}} \; {\MRup_{i}^{j}}]$, and 
$[{\GRlo_{i}^{j}} \; {\GRup_{i}^{j}}]$, 
where corresponding response time.
In this model, we have already known the length of CPU, memory, and GPU $CL_{i}^{j}$, $ML_{i}^{j}$ and $GL_{i}^{j}$. Meanwhile, the CPU and memory response time lower bounds $\CRlo_{i}^{j}$ and $\MRlo_{i}^{j}$ are known to be equal to the length of CPU, memory $CL_{i}^{j}$ and $ML_{i}^{j}$, because their shortest response time are the execution time in one CPU core and memory interface without waiting, blocking or preemption. However, we do not know their response time upper bounds because in their execution, waiting, blocking and preemption may happen. For the GPU response time, it depends on the number of SMs assigned to the GPU kernel. 
}

\subsection{Federated Scheduling for GPU Segments}

%In this work, we focus on the parallel real-time scheduling problem on a GPU comprised of $N_{SM}/2$ physical SMs modeled as $N_{SM}$ virtual SMs and a taskset with $n$ tasks.
%We consider the sporadic real-time tasks, where the $jth$ GPU segment in task $i$ has an \defn{implicit deadline} $GD_i^{j}$, which is equal to its period $GT_i^{j}$. 

For executing the GPU segments of the $n$ tasks on the shared GPU with $2{\GN}$ virtual SMs (i.e., ${\GN}$ physical SMs), we propose to generalize \defn{federated scheduling}~\cite{FS}, a scheduling paradigm for parallel real-time tasks on CPU, to scheduling parallel GPU segments. The key insight of federated scheduling is to calculate and assign the minimum number of dedicated resources needed for each parallel task to meet its deadline. 

Specifically, we allocate $2\GN_i$ dedicated virtual SMs to each task $\tau_i$, such that its GPU segment $G_i^j$ can start executing immediately after the completion of the corresponding memory copy $\ML_i^{2j}$. In this way, the mapping and execution of GPU kernels to SMs are explicitly controlled by the platform via the persistent thread and workload pinning interfaces, so the effects caused by the black-box internal scheduler of a GPU are minimized. Additionally, tasks do not need to compete for SMs, so there is no blocking time on the non-preemptive SMs. Furthermore, via the self-interleaving technique, we enforce that GPU kernels do not share any physical SMs. Therefore, the interference between different GPU segments is minimized, and the execution times of GPU segments are more predictable.

{\color{red} Move to the earlier section (need to make sure notations are consistent): \\
Since the GPU kernels are embarrassingly parallel workloads, as discussed in Section~\ref{kernelmodel}, a GPU segment in task $\tau_i$ where $1\le i\le n$ with multiple kernels can be modeled similarly using the classic \emph{parallel synchronous task model}. We model the \defn{total work} $\GW_{i}^{j}$ of a kernel $G_{i}^{j}$ using the total execution time of the kernel on a single SM in isolation, i.e., without any interleaving. The overhead of launching kernel is denoted as \defn{critical-path overhead} $\GL_{i}^{j}$.
Therefore, the total work $\GW_i^{j}$ of the GPU kernels in task $\tau_i$ is $\GW_i^{j}$ and the critical-path overhead is $\GL_i^{j}$. The \defn{utilization} $u_i^{j}$ of this GPU segment is defined as $u_i = \GW_i^{j}/T_i^{j}$. To capture a GPU segment's execution on self-interleaved SMs, we define the total execution time of this GPU segment on a single SM with two virtual SMs interleaved with itself as the \defn{total virtual work} $\GW_i^{j} \alpha_i^j$, where the $\alpha_i^j$ is defined as the \defn{interleaved execution ratio} of this segment.
%Finally, we define the \defn{maximum interleaved execution ratio} of a task set $\tau$ as $\alpha = \max_i \alpha_i$. 

%GPU kernel launch overhead models the data copy from memory/L2 to the SM, which happens inside a GPU system. The worst overhead happens when the data is copied to the execution unit in SM for one execution and then copied back to the GPU memory.
}

%The above real-time GPU system model based on our proposed virtual SM model with persistent threads technique enables us to calculate how many dedicated virtual SMs are required by a GPU segment to meet its implicit deadline and to explicitly partition virtual SMs to tasks based on their needs. 

In summary, each task $\tau_i$ is assigned with $2\GN_i$ dedicated virtual SMs where each of its GPU segments self-interleaves and has an interleaved execution ratio $\alpha_i^j$. In Section~\ref{algo}, we will present the algorithm that determines the SM allocation to tasks. Here, for a given allocation, we can easily extend the formula in Section~\ref{kernelmodel} to obtain the following lemma for calculating the response time $\GR_i^j$ of a GPU segment $G_i^j$.

%\begin{lemma}
%\label{lem:ncores}
%\textbf{(From \cite{FS})}
%If the GPU segment has a total virtual work $GW'_i^{j}$ and a critical-path overhead of $GLL_i^{j}$, then it is schedulable and can meet its implicit deadline $GD_i^{j}$ with $GN_i$ dedicated virtual SMs, where $GN_i \geq \frac{GW'_i^{j}-GLL_i^{j}}{GD_i^{j}-GLL_i^{j}} $.
%\end{lemma}
\begin{lemma}
\label{lem:ncores}
If the GPU segment $G_i^j$ has a total work in range $[\GWlo_i^{j}, \GWup_i^{j}]$, a worst-case critical-path overhead of $\GLup_i^{j}$ and an interleaved execution ratio $\alpha_i^j$, then when running on $2\GN_i$ dedicated virtual SMs, its response time is in $[\GRlo_i^{j}, \GRup_i^{j}]$ where
\[
\GRlo_i^j = \frac{\GWlo_i^{j}\alpha_i^j}{2\GN_i}, \mbox{\ and \ }
\GRup_i^j = \frac{\GWup_i^{j}\alpha_i^j - \GLup_i^{j}}{2\GN_i}+\GLup_i^{j}.
\]
\end{lemma}
\begin{proof}
The lower bounds $\GRlo_{i}^{j}$ is the shortest execution time of this GPU segment on $2GN_i$ virtual SMs. In the best case, there is no critical-path overhead and the minimum total virtual work $\GWlo_i^{j}\alpha_i^j$ is executed in full parallelism on $2GN_i$ virtual SMs, which gives the formula of $\GRlo_{i}^{j}$.
In the worst case, the maximum total virtual work is $\GWup_i^{j}\alpha_i^j$, and the maximum critical-path overhead $\GLup_i^{j}$ captures the maximum overhead of launching the kernel. Since $\GLup_i^{j}$ is a constant overhead and is not affected by self-interleaving and multiple virtual SMs, we do not need to apply the interleaved execution ratio $\alpha_i^j$ to $\GLup_i^{j}$. After deducting the critical-path overhead, the remaining GPU computation is embarrassingly parallel on $2GN_i$ virtual SMs, which results the formula of $\GRup_{i}^{j}$. 
\end{proof}


Note that the above Lemma~\ref{lem:ncores} calculates both the lower and upper bounds on the response time of GPU segment $G_i^j$, because both bounds are needed when analyzing the total response time of task $\tau_i$. {\color{red} Talk about platform support for ensuring lower bound?}

%Note that the above Lemma~\ref{lem:ncores} for calculating the minimum number of virtual SMs is similar to the Theorem 2 from previous work~\cite{FS} for calculating the minimum number of CPUs. Therefore, we propose the real-time GPU scheduling algorithm as follows.
%Given a task set $\tau$, our algorithm first uses Lemma~\ref{lem:ncores} to calculate the number of virtual SMs $m_i$ assigned to GPU segments in each task $\tau_i$. 

%then our algorithm \emph{admits} the task set; otherwise, our algorithm declares the task set as unschedulable. Then the GPU response upper bounds $\GRup_{i}^{j}$ is the deadline $GD_{i}^{j}$ and the lower bounds $\GRlo_{i}^{j}$ is the shortest execution time of this GPU segment with $GN_i$ virtual SMs.

To ensure that tasks do not share SMs, the total number of virtual SMs assigned to all tasks must be no more than the number of available virtual SMs, i.e., $\sum_i \GN_i \le \GN$; otherwise, the task set is unschedulable. During runtime execution of schedulable task sets, our platform will generate $2\GN_i$ persistent threads blocks for each GPU segment of task $\tau_i$ to execute on its assigned $2\GN_i$ virtual SMs. 


%Federated scheduling has been proved to have a \defn{capacity augmentation bound} of 2 for CPU tasks, meaning that given $m$ cores federated scheduling can guarantee schedulability to any task set $\tau$ on $m$ CPU cores as long as it satisfies:
%(1) the total utilization of the task set is no more than half of the total available cores, i.e., $\sum{u_i} \le m/2$; 
%(2) for each task, the critical-path overhead is less than half of its deadline, i.e., $L_i < D_i/2$. Based on our virtual SM model, we can easily prove that our generalized federated scheduling algorithm for real-time GPU task has a capacity augmentation bound of $\alpha$ with respect to any non-interleaved optimal scheduler, where $\alpha$ is the maximum interleaved execution ratio and is at most 2.


\subsection{Background on Multi-Segment Self-Suspension}

{\color{red} need to change $C$ to $L$ to be consistent.}

In the multi-segment self-suspension system model, a task is expressed as:
\begin{equation}
\tau_i = \big( (C_{i}^{0}, S_{i}^{0}, C_{i}^{1}, ..., S_{i}^{m_{i}-2}, C_{i}^{m_{i}-1}), D_{i}, T{i} \big)
\label{eq:self-suspension model}
\end{equation}
where ${m_{i}}$ is the number of computation and ${m_{i}-1}$ is the number of suspension segments in the task $\tau_i$. And $C_{i}^{j}$ and $S_{i}^{j}$ are the $j th$ computation segment and suspension segment in the task $\tau_i$. $[\Slo_{i}^{j} \; \Sup_{i}^{j}]$ are the corresponding suspension upper bounds and lower bounds.
According to the schedulability analysis in \cite{huang2015schedulability}, the workload function $W_{i}^{h}(t)$ of the $hth$ computation segment in task $i$ in an interval length $t$ can be expressed as:
\begin{equation}
\begin{aligned}
W_{i}^{h}(t) &= \sum_{j=h}^{l}C_{i}^{j \bmod m_{i}}+ \\
&min(C_{i}^{(l+1) \bmod  m_{i}}, t-\sum_{j=h}^{l}(C_{i}^{j \bmod  m_{i}}+S_{i}^{j}))
\end{aligned}
\label{eq:workload function}
\end{equation}
where $l$ is the maximum integer satisfying the following condition:
\begin{equation}
\begin{aligned}
\sum_{j=h}^{l}(C_{i}^{j \bmod  m_{i}}+S_{i}^{j}) \leq t
\end{aligned}
\label{eq:workload function}
\end{equation}
and

\begin{equation}
S_{i}^{j} = \left\{
             \begin{array}{lr}
             {\Slo}_{i}^{j \bmod m_{i}} & \mbox{if\ } j \bmod m_{i} \neq (m_{i}-1) \\
             T_{i}-D{i} & \mbox{else if\ } j \leq m_{i}\\
             T_{i}-(C_{i}+\Slo_{i}) &  \mbox{otherwise}
             \end{array}
\right.
\end{equation}

The maximum workload function $W_{i}(t)$ of task $i$ in an interval length $t$ is:
\begin{equation}
W_{i}(t) = max_{h_{i}\in[0,m_{i}-1]}{W_{i}^{h_{i}}(t)}
\label{eq:workload function}
\end{equation}

For the worst-case response time $R_{k}^{j}$ of subtask $j$ in task $k$, denotes the smallest value satisfying the following recurrence:
\begin{equation}
R_{k}^{j} = C_{k}^{j} + \sum_{\tau_{i}\in hp(k)}W_{i}(R_{k}^{j})
\label{eq:workload function}
\end{equation}
where $W_{i}(t)$ is the maximum workload function and $hp(k)$ denotes the set of the tasks with higher priority than task $k$.

The worst-case response time $R_{k}$ of task $k$ is:
\begin{equation}
R_{k} = min \left\{
             \begin{array}{lr}
             R_{k}=C_{k} + \Sup_{i} + \sum_{\tau_{i}\in hp(k)}W_{i}(R_{k}) \\
             \Sup_{i} + \sum_{j=0}^{m_{k}-1}R_{k}^{j} \\
             \end{array}
\right.
\label{eq:workload function}
\end{equation}



\subsection{Fixed-Priority Scheduling for Memory-Copy Segments with Self-Suspension and Blocking}

After getting the GPU response time upper bounds and lower bounds $[\GRlo_{i}^{j} \; \GRup_{i}^{j}]$, a fixed priority real-time scheduling algorithm for the CPU and memory segments in the hard deadline parallel GPU tasks is proposed.

Based on the real-time scheduling model and looking the tasks from the CPU (or memory or GPU) perspective, the tasks are “self-suspension style" tasks \cite{chen2019many} where the CPU codes are the computation segments and the memory and GPU segments are the suspension segments. Compared with classic self-suspension tasks, this “self-suspension style" model has following difference. 1. The suspension part is made of memory copy and GPU segments. 2. The suspension in one task be be blocked by suspension in other tasks because the suspension contains the non-preemptive memory copy. 3. The execution time of suspension segment is not equal to the length of the suspension segment because the memory copies in the suspension segment may be blocked or do not has the access to the memory interface when it is ready to execution. Based on the state-of-the-art classic suspension schedulability analysis \cite{huang2015schedulability}, we propose a schedulability analysis for this kind of “self-suspension style" system. This schedulability analysis is not only limited to CPU-memory-GPU system, but also can be applied to other heterogeneous computing systems like CPU-memory-FPGA, CPU-memory-TUP systems.

Based on above state-of-the-art analysis on classic suspension tasks, we develop the schedulability analysis for this “self-suspension style" model. After the GPU federated scheduling, we have known the GPU response time upper bounds and lower bounds $[\GRlo_{i}^{j} \; \GRup_{i}^{j}]$. Meanwhile, we also know the CPU and memory execution time lower bounds $\CRlo_{i}^{j}$ and $\MRlo_{i}^{j}$ because the response time lower bound is equal to the length CPU and memory segments $CL_{i}^{j}$ and $ML_{i}^{j}$, which means that the CPU and memory segments are executed immediately when they are ready and are not preempted during execution.

We first consider the memory segments and calculate the response time upper bounds of each memory segment $\MRup_{i}^{j}$. Looking from the memory perspective, the memory itself is the "non-preemptive computation" and the CPU and GPU are the "suspension". Therefore, the workload function $MW_{i}^{h}(t)$ of the $hth$ memory segment in task $\tau_i$ can be expressed as:
\begin{equation}
\begin{aligned}
&MW_{i}^{h}(t) = \sum_{j=h}^{l}ML_{i}^{j \bmod  m_{i}}+ 
min(\\
&ML_{i}^{(l+1) \bmod  m_{i}}, t-\sum_{j=h}^{l}(ML_{i}^{j \bmod  m_{i}}+S_{i}^{j}))
\end{aligned}
\label{eq:workload function}
\end{equation}

where $l$ is the maximum integer satisfying the following condition:
\begin{equation}
\begin{aligned}
\sum_{j=h}^{l}(ML_{i}^{j \bmod  m_{i}}+S_{i}^{j}) \leq t
\end{aligned}
\label{eq:workload function}
\end{equation}
and

\begin{equation}
S_{i}^{j} = \left\{
             \begin{array}{lr}
             \CLlo_{i}^{j \bmod m_{i}} + \GLlo_{i}^{j \bmod m_{i}}& \mbox{if\ } j \bmod m_{i} \neq (m_{i}-2) \\
             T_{i}-D{i} & \mbox{else if\ } j \leq m_{i}\\
             T_{i}-(ML_{i}+{\CLlo_{i}}+{\GLlo_{i}}) &  \mbox{otherwise\ }
             \end{array}
\right.
\end{equation}



The maximum workload function $MW_{i}(t)$ of task $i$ in an interval length $t$ is:
\begin{equation}
MW_{i}(t) = max_{h_{i}\in[0,m_{i}-2]}{MW_{i}^{h_{i}}(t)}
\label{eq:workload function}
\end{equation}


For the worst-case response time $MR_{k}^{j}$ of memory segment $j$ in task $k$, denotes the smallest value satisfying the following recurrence. $max(ML_{\tau_{i}\notin hp(k)}^{j})$ denotes the blocking from lower priority memory copy.
\begin{equation}
\MRup_{i}^{j} = ML_{k}^{j} + \sum_{\tau_{i}\in hp(k)}MW_{i}(\MRup_{i}^{j})+max(ML_{\tau_{i}\notin hp(k)}^{j})
\label{eq:workload function}
\end{equation}

\subsection{Fixed-Priority Scheduling for CPU Segments}

The schedulability analysis is described as follows. 
After the upper bound response time of memory, we calculate the full task response time. Looking from the CPU perspective, the CPU segment itself is  the ”computation” and the memory and GPU are the ”suspension”. Therefore, the workload function $CW_{i}^{h}(t)$ of the $hth$ CPU segment in task $\tau_i$ can be expressed as:
\begin{equation}
\begin{aligned}
&CW_{i}^{h}(t) = \sum_{j=h}^{l}CL_{i}^{j \bmod  m_{i}}+ 
min(\\
&CL_{i}^{(l+1) \bmod  m_{i}}, t-\sum_{j=h}^{l}(CL_{i}^{j \bmod  m_{i}}+(ML+GL)_{i}(j)))
\end{aligned}
\label{eq:workload function}
\end{equation}

where $l$ is the maximum integer satisfying the following condition:
\begin{equation}
\begin{aligned}
\sum_{j=h}^{l}(CL_{i}^{j \bmod  m_{i}}+S_{i}^{j}) \leq t
\end{aligned}
\label{eq:workload function}
\end{equation}
and

\begin{equation}
S_{i}^{j} = \left\{
             \begin{array}{lr}
             \MLlo_{i}^{j \bmod m_{i}} + \GLlo_{i}^{j \bmod m_{i}} & \mbox{if\ } j \bmod m_{i} \neq (m_{i}-1) \\
             T_{i}-D{i} &  \mbox{else if\ } j \leq m_{i}\\
             T_{i}-(CL_{i}+\MLlo_{i} + \GLlo_{i}) &  \mbox{otherwise\ }
             \end{array}
\right.
\end{equation}

The maximum workload function $CW_{i}(t)$ of task $i$ in an interval length $t$ is:
\begin{equation}
CW_{i}(t) = max_{h_{i}\in[0,m_{i}-1]}{CW_{i}^{h_{i}}(t)}
\label{eq:workload function}
\end{equation}

For the worst-case response time $CR_{k}^{j}$ of CPU segment $j$ in task $k$, denotes the smallest value satisfying the following recurrence:
\begin{equation}
\CRup_{k}^{j} = CL_{k}^{j} + \sum_{\tau_{i}\in hp(k)}CW_{i}(\CRup_{k}^{j})
\label{eq:workload function}
\end{equation}

Then the worst-case response time $R_{k}$ of task $k$ is:
\begin{equation}
R_{k} = min \left\{
             \begin{array}{lr}
             CL_{k} + \MRup_{i} + \GRup_{i} + \sum_{\tau_{i}\in hp(k)}CW_{i}(R_{k}) \\
             \MRup_{i} + \GRup_{i} + \sum_{j=0}^{M_{k}-1}\CRup_{k}^{j} \\
             \end{array}
\right.
\label{eq:workload function}
\end{equation}

\subsection{RT-GPU Scheduling Algorithm}

The full procedure of scheduling GPU tasks can be described as follows: (1) Grid search a federated scheduling for the GPU codes and calculate the GPU segment response time $[\GRlo_{i}^{j} \; \GRup_{i}^{j}]$, details in Section \ref{sec:schedule}.4. (2) The CPU segments and memory copy segments are scheduled by fixed priority scheduling. (3) If all the tasks can meet the deadline, then they are schedulable and otherwise go back to step (1) to grid search for a next federated scheduling. This schedulability test for hard deadline parallel GPU tasks can be summarized in Algorithm \ref{Algorithm: schedulability_test}.
{\color{red} add more detailed explanation. Change the code style.}

{\color{red} 
This proposed scheduling algorithm is not limited to the fixed configuration of "CPU-Memory-GPU-Memory-CPU-...". 
It can be applied to any combinations of CPU, memory and GPU segments in any orders. }

\begin{algorithm}
\caption{Fixed Priority Self-Suspension with Grid Searched Federated Scheduling} 
\label{Algorithm: schedulability_test}
\raggedright{\bf {Input Variables:}}\\
\raggedright{\textbf{\quad} Parameters for tasks and sub-tasks: in section 5.1 and 5.2}\\
\raggedright{\bf {Output Variables:}}\\
\raggedright{\textbf{\quad} Scheduability, Federated scheduling: $m^{SM}_{i}$} \\
\raggedright{\bf {Steps:}}\\
\textbf{void} main()\{ \\
 
\raggedright{\textbf{\quad}\textit{\small{//\textbf{1:} GPU kernel federated scheduling grid search:}}}\\
\raggedright{\textbf{\quad} \textbf{for} $m^{SM}_{1}$ = 1, ..., $M$ \textbf{do}}\\
\raggedright{\textbf{\quad \quad} \textbf{for} $m^{SM}_{...}$ = 1, ..., $M$ \textbf{do}}\\ 
\raggedright{\textbf{\quad \quad \quad} \textbf{for} $m^{SM}_{n}$ = 1, ..., $M$ \textbf{do}}\\ 
\raggedright{\textbf{\quad \quad \quad \quad} \textit{\small{//\textbf{2:} Calculate GPU sub-task deadlines and remainning}}} \\
\raggedright{\textbf{\quad \quad \quad \quad} \textit{\small{copy deadlines under current kernel federated scheduling:}}} \\
\raggedright{\textbf{\quad \quad \quad \quad} \textbf{if} ($\sum^{n}_{i=1}{GN_{i}} \leq N_{SM}$) \textbf{then}}\\
\raggedright{\textbf{\quad \quad \quad \quad\quad} $GD_{i}^{j} = \lceil \frac{GW_{i}^{j}+(GN_{i}-1)GLL_{i}{j}}{m^{SM}_{i}} \rceil$ }\\
\raggedright{\textbf{\quad \quad \quad \quad\quad} $\GRup_{i}^{j}$ = $GD_{i}^{j}$ }\\
\raggedright{\textbf{\quad \quad \quad \quad\quad} $\GRlo_{i}^{j}$ = shortest execution time of $\GL_{i}^{j}$}\\
\raggedright{\textbf{\quad \quad \quad \quad} \textit{\small{//\textbf{3:} Calculate the memory copy execution upper bound}}} \\
\raggedright{\textbf{\quad \quad \quad \quad} \textbf{for all} i = 1, ..., n; j = 0, ..., $m_{i}-2$ \textbf{do}}\\

\raggedright{\textbf{\quad \quad \quad \quad \quad} Calculate the memory segment response time}\\

\raggedright{\textbf{\quad \quad \quad \quad \quad} upper bounds with E.q.(10) - (14)}\\

\raggedright{\textbf{\quad \quad \quad \quad \quad} Calculate the CPU segment and full task}\\

\raggedright{\textbf{\quad \quad \quad \quad \quad} response time upper bounds with E.q.(15) - (20)}\\

\raggedright{\textbf{\quad \quad \quad \quad} \textbf{then return} pass schedulability test and $m^{SM}_{i}$ }\\ 
\raggedright{\textbf{\quad \quad \quad \quad} \textbf{end for all}}\\ 
\raggedright{\textbf{\quad \quad \quad} \textbf{end for}}\\ 
\raggedright{\textbf{\quad \quad} \textbf{end for}}\\ 
\raggedright{\textbf{\quad} \textbf{end for}}\\ 
\raggedright{ \textbf{return} fail schedulability test\}}
\end{algorithm}





